Fine-grained Distributed Data Plane Verification with Intent-based Slicing

Data plane verification has grown into a powerful tool to ensure network correctness. However, existing methods with monolithic models have memory requirements tied to network sizes, and the existing method of scaling out is too limited in expressiveness to capture practical network features. In this paper, we describe Scylla, a general data plane verifier that provides fine-grained scale-out without the need for a monolithic network model. Scylla creates models for what we call intent-based slices, each of which is constructed at the rule-level granularity with only enough to verify a given set of intents. The sliced models are retained and incrementally updated in memory across a distributed compute cluster in response to network updates. Our experiments show that Scylla makes the scaling problem more granular -- tied to the size of the intent-based slices rather than that of the overall network. This enables Scylla to verify large, complex networks in minimum units of work that are significantly smaller (in both memory and time) than past techniques, enabling fast scale-out verification with minimal resource requirement.

==> Makefile <==
#
# Makefile
#

PDF = scylla.pdf

all: ${PDF}

%.pdf: %.tex # acmart.cls ACM-Reference-Format.bst
	pdflatex $(notdir $<)
	- bibtex $(notdir $(basename $<))
	pdflatex $(notdir $<)
	pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
		do pdflatex $(notdir $<); done

# %.cls: %.ins %.dtx
# 	pdflatex $<

# .PRECIOUS: acmart.cfg acmart.cls

docclean:
	$(RM) *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.xdv *.fdb_latexmk *.fls *.bak *.tmp \
	*.synctex.gz

clean: docclean
	# $(RM) acmart.cls

distclean: clean
	$(RM) ${PDF}

.PHONY: all docclean clean distclean

